Graph Attention Convolutional U-NET: A Semantic Segmentation Model for Identifying Flooded Areas

The increasing impact of human-induced climate change and unplanned urban constructions has increased flooding incidents in recent years. Accurate identification of flooded areas is crucial for effective disaster management and urban planning. While few works have utilized convolutional neural networks and transformer-based semantic segmentation techniques for identifying flooded areas from aerial footage, recent developments in graph neural networks have created improvement opportunities. This paper proposes an innovative approach, the Graph Attention Convolutional U-NET (GAC-UNET) model, based on graph neural networks for automated identification of flooded areas. The model incorporates a graph attention mechanism and Chebyshev layers into the U-Net architecture. Furthermore, this paper explores the applicability of transfer learning and model reprogramming to enhance the accuracy of flood area segmentation models. Empirical results demonstrate that the proposed GAC-UNET model, outperforms other approaches with 91\% mAP, 94\% dice score, and 89\% IoU, providing valuable insights for informed decision-making and better planning of future infrastructures in flood-prone areas.

==> extra.tex <==

\begin{table}[ht]
	\centering
	\caption{Comparison of dice loss vs BCE loss and comparison of proposed approach against baselines.}
	\begin{tabu}{l | *{4}{X[c]}}
	\toprule
 	\quad \quad Approach & Loss & IoU & Dice Score & mAP  \\
	\midrule
 	\multirow {2}{*}{Convolutional U-NET} & BCE &  0.71 & 0.82 & 0.75\\
 	 & Dice & 0.73 & 0.83 & 0.76\\
 	\midrule
    \multirow {2}{*}{Efficient Neural Network} & BCE & 0.69 & 0.79 & 0.76\\
     & Dice &  0.71 & 0.82 & 0.78\\
 	\midrule
    Graph Attention Convolutional U-NET & BCE & 0.79 & 0.83 & 0.77\\
 	\textit{(Our proposed model)} & Dice & \textbf{0.89} & \textbf{0.94} & \textbf{0.91}\\
	\bottomrule
	\end{tabu}

	\label{tab:gat-results}
\end{table}


\begin{table}[ht]
	\centering
	\caption{Comparison of transfer learning and model reprogramming on Segformer.}
	\begin{tabu}{l | *{3}{X[c]}}
	\toprule
 	\quad \quad Approach & IoU & Dice Score & mAP  \\
	\midrule
 	Traditional Training &  0.67 & 0.79 & 0.72\\
 	Transfer Learning & \textbf{0.76} & \textbf{0.86} & \textbf{0.82}\\
 	Model Reprogramming & 0.69 & 0.80 & 0.75\\
	\bottomrule
	\end{tabu}

	\label{tab:transfer-results}
\end{table}

